Number theory casting a look at the mirror

In this work, we give a purely analytic introduction to the phenomenon of mirror symmetry for quintic threefolds via classical hypergeometric functions and differential equations for them. Starting with a modular map and recent transcendence results for its values, we regard a mirror map $z(q)$ as a concept generalizing the modular one. We give an alternative approach demonstrating the existence of non-linear differential equations for the mirror map, and exploit both an elegant construction of Klemm-Lian-Roan-Yau and the Ax theorem to prove that the Yukawa coupling $K(q)$ does not satisfy any algebraic differential equation of order less than 7 with coefficients from $\mathbb{C}(q)$.

==> mfpic.tex <==
%%%
%%%  File: mfpic.tex
%%%
% preliminary version of macros.
\chardef\oldatcatcode=\catcode`@
\catcode`@=11
\immediate\write16
  {mfpic version 0.2.9 alpha  Thu 11 August 1994}%
% local declarations:
\wlog {mfpic: local declarations}%
\newwrite\@outx
\newread\@graphx
\newcount\@gcode
\newbox\@labeledgraph
\newbox\@temp
\wlog {mfpic: internal dimension parameters}%
\newdimen\@graphwd
\newdimen\@graphleft
\newdimen\@graphht
\newdimen\@graphdp
\newdimen\@centerskip
\newdimen\@labeltemp
\def\do@ptparam#1#2{%
  \def\@ptparami[##1]{\csname#1\endcsname[##1]}%
  \def\@ptparamii{\csname#1\endcsname[#2]}%
  \def\@ptparamiii{%
    \ifx[\nchr \expandafter\@ptparami
    \else \expandafter\@ptparamii\fi}%
  \futurelet\nchr\@ptparamiii}%
% dimension parameters:
\wlog {mfpic: user's dimension parameters}%
\newdimen\mfpicunit
\mfpicunit=1pt
\newdimen\pointsize
\newif\ifpointfilled\pointfilledtrue
\newdimen\shadespace
\newdimen\hatchspace
\newdimen\headlen
\newdimen\axisheadlen
\newdimen\hashlen
\newdimen\dashlen
\newdimen\dashspace
% default settings:
\pointsize=2pt
\shadespace=1pt
\hatchspace=3pt
\headlen=3pt
\axisheadlen=5pt
\hashlen=4pt
\dashlen=4pt
\dashspace=4pt
% standard setting macros:
\def\darkershade{%
  \multiply\shadespace by 5
  \divide\shadespace by 6}%
\def\lightershade{%
  \multiply\shadespace by 6
  \divide\shadespace by 5}%
\def\dashlineset{%
  \dashlen=4pt
  \dashspace=4pt}%
\def\dotlineset{%
  \dashlen=1pt
  \dashspace=2pt}%
% direct output to Metafont file:
\def\mfcmd#1{%
  \immediate\write\@outx{#1}%
  \ignorespaces}%
% pen size setting:
\def\@pickup{%
  \mfcmd{pickup pencircle scaled penwd;}}%
\def\pen#1{%
  \mfcmd{interim penwd:=#1;}%
  \@pickup}%
% arrowhead shape setting:
\def\headshape#1#2#3{%
  \mfcmd{%
    interim hdwdr:=#1;
    interim hdten:=#2;
    hfilled:=#3;}}%
% Prefix commands:
% routines to select drawing (of paths) :
\newif\if@drawing\@drawingtrue
\newif\if@path\@pathfalse
\newif\if@dodraw\@dodrawtrue
\newif\if@connect\@connectfalse
\newif\if@doconnect\@doconnectfalse
\def\@doreset{%
  \@dodrawtrue
  \if@connect
     \@drawingfalse
     \@pathtrue
     \@doconnecttrue
  \else
     \@drawingtrue
     \@pathfalse
     \@doconnectfalse
   \fi
  \ignorespaces}%
\def\@checkpath#1#2{%
  \if@drawing
    \if@path
      \mfcmd{#1}%
    \else
      \mfcmd{#2}%
    \fi
  \fi}%
\def\@draw#1{%
  \@checkpath{drawnpath}{safedraw}%
  \mfcmd{\if@connect\else ( \fi
    \if@doconnect transformed ztr)--( \fi #1
    \if@connect \else ) transformed ztr; \fi}%
  \@doreset}%
% store following mfpic path in MF path variable #1:
\def\store#1{\@mfcmd{path #1; #1:=}\@drawingfalse}%
% shading, hatching, filling, and erasing:
\def\@shade[#1]{\mfcmd{shadepath(#1)}\@drawingfalse}%
\def\shade{\do@ptparam{@shade}{\the\shadespace}}%
\def\@hatch[#1]{\mfcmd{hatchpath(#1)}\@drawingfalse}%
\def\hatch{\do@ptparam{@hatch}{\the\hatchspace}}%
\def\fill{\mfcmd{safefill}\@drawingfalse}%
\def\white{\mfcmd{safeunfill}\@drawingfalse}%
% arrowheads:
\def\@arrow{%
  \@checkpath{}{trash:=}%
  \mfcmd{headpath(\@hlength,\@hrotate,\@hbackset)}%
  \@pathtrue}%
\def\@checkchar#1#2{%
  \ifx#1l\gdef\@hlength{#2}\else
  \ifx#1r\gdef\@hrotate{#2}\else
  \ifx#1b\gdef\@hbackset{#2}\fi\fi\fi}%
\def\@arrowthree[#1#2]{\@checkchar{#1}{#2}\@arrow}%
\def\@arrowtwo[#1#2]{%
  \@checkchar{#1}{#2}%
  \do@ptparam{@arrowthree}{WW}}%
\def\@arrowone[#1#2]{%
  \gdef\@hlength{\the\headlen}%
  \gdef\@hrotate{0}%
  \gdef\@hbackset{0pt}%
  \@checkchar{#1}{#2}%
  \do@ptparam{@arrowtwo}{ZZ}}%
\def\arrow{\do@ptparam{@arrowone}{YY}}%
% outline, dotted lines, and closed paths:
\def\draw{%
  \if@dodraw\@checkpath{}{trash:=}%
    \mfcmd{drawnpath}\fi
  \@drawingfalse\@dodrawfalse}%
\def\@dotted[#1,#2]{%
  \if@dodraw\@checkpath{}{trash:=}%
    \mfcmd{dotted(#1,#2)}\fi
  \@drawingfalse\@dodrawfalse}%
\def\dotted{%
  \do@ptparam{@dotted}%
    {\the\dashlen,\the\dashspace}}%
\def\closed{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{closedpath}%
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
\def\bclosed{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{bclosedpath}%
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
\def\sclosed{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{sclosedpath}%
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
\def\cbclosed{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{cbclosedpath}%
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
% reversing orientation of paths:
\def\reverse{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{\if@doconnect transformed ztr)--(\fi reverse}%
  \@doconnectfalse
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
% connecting open figures:
\def\connect{\@checkpath{drawnpath}{safedraw}%
  \mfcmd{(}%
  \bgroup
    \@connecttrue\@doconnectfalse
    \if@drawing\@dodrawfalse\fi
    \@drawingfalse}%
\def\endconnect{%
    \mfcmd{) transformed ztr;}%
    \@doconnectfalse\@connectfalse
  \egroup
  \@doreset}%
% rotating a path:
\def\rotate#1{%
  \@checkpath{drawnpath}{safedraw}%
  \mfcmd{rotatedpath(#1)}%
  \@pathtrue
  \if@drawing\@dodrawfalse\fi
  \@drawingfalse}%
% Affine transforms of the MF _coordinate system_ :
% grouping macros that enable nested coordinate systems:
\def\coords{\mfcmd{bcoords;}}%
\def\endcoords{\mfcmd{ecoords;}}%
% macro that applies a nominated MF affine transformer:
\def\applyT#1{\mfcmd{apply_t(#1);}}%
% specific transform macros for MF coordinates;
% see _The METAFONTbook_ for most of these.
\def\rotates#1{\applyT{rotated #1}}%  degrees
\def\rotatesaround#1#2{\applyT{rotatedaround(#1,#2)}}%  point, degrees.
\def\reflectsabout#1#2{\applyT{reflectedabout(#1,#2)}}%  line #1 -- #2.
\def\shifts#1{\applyT{shifted #1}}%  pair.
\def\scales#1{\applyT{scaled #1}}%  same scaling in X and Y directions.
\def\xscales#1{\applyT{xscaled #1}}%  scale only X.
\def\yscales#1{\applyT{yscaled #1}}%  scale only Y.
\def\zscales#1{\applyT{zscaled #1}}%  complex multiplication of points.
\def\xslants#1{\applyT{xslanted #1}}%  skew in X direction by a multiple of Y coord.
\def\yslants#1{\applyT{yslanted #1}}%  skew in Y direction by a multiple of X coord.
\def\zslants#1{\applyT{zslanted #1}}%  see `graphbase.mf'.
\def\xyswaps#1{\applyT{xyswapped #1}}%  reflect in line Y=X.
\def\boosts#1{\applyT{boosted #1}}%  special relativity boost.
% end Prefix commands.
% open and close MF graphs file:
\def\opengraphsfile#1{%
  \@gcode=0
  \immediate\openout\@outx=#1.mf
  \openin\@graphx=#1.tfm
  \ifeof\@graphx
    \immediate\write16
      {No file #1.tfm.}%
    \font\@graph=dummy\relax
  \else
    \font\@graph=#1\relax
  \fi
  \closein\@graphx
  \immediate\write16
    {mfpic: Don't forget to process #1.mf!}%
  \immediate\write16
    { Then reprocess this file.}%
  \mfcmd{if unknown mode: mode:= localfont; fi}%
  \mfcmd{if unknown mag: mag:=\number\mag/1000; fi}%
  \mfcmd{if unknown graphbase: input graphbase; fi}%
  \mfcmd{gcode:=\number\@gcode;}%
  % set global defaults:
  \headshape{1}{1}{false}%
  \mfcmd{interim penwd:=0.5pt;}%
  \mfcmd{}}%
\def\closegraphsfile{%
  \mfcmd{}%
  \mfcmd{end.}%
  \immediate\closeout\@outx}%
% percent and sharp signs for MF file:
\def\mf@gobble#1{}%
\def\mf@p{\expandafter\mf@gobble\string\%}%
\def\mf@s{\expandafter\mf@gobble\string\#}%
% for reading \@mfpic:
\global\font\@tcurr=\fontname\font\relax
\nullfont
% beginning mfpic environment:
\def\@mfpic#1#2#3#4#5#6%
{%
 % set up TeX
 \leavevmode
 \bgroup
  \parfillskip0pt plus1fill
  % conversion (local) :
  \def\@xconv##1{%
    \global\advance##1 by -#3\mfpicunit
    \global ##1 = #1 ##1}%
  \def\@yconv##1{%
    \global\advance##1 by -#5\mfpicunit
    \global ##1 = -#2 ##1}%
  % set up graph box:
  \global\advance\@gcode1
  \global\@graphwd=#4\mfpicunit
  \@xconv\@graphwd
  \@graphht=#6\mfpicunit
  \@yconv\@graphht
  \@graphleft=0pt
  \@graphdp=0pt
  \global\setbox\@labeledgraph=
    \vtop{\noindent\@graph\char\@gcode}%
  % set up Metafont file:
  \mfcmd{}%
  \mfcmd{unitlen:=\the\mfpicunit\mf@s;}%
  \mfcmd{xscale:=#1*unitlen; yscale:=#2*unitlen;}%
  \mfcmd{xneg:=#3; xpos:=#4;}%
  \mfcmd{yneg:=#5; ypos:=#6;}%
  \mfcmd{beginchar
    (incr gcode,
     (xpos-xneg)*xscale,
     (ypos-yneg)*yscale,
     0);}%
  \mfcmd{initpic;}%
  % the (MF based) drawing macros:
  % Metafont title
  \def\mftitle##1{%
    \mfcmd{"##1";}}%
  % allow MF path ##1 to be shaded, connected, etc:
  \def\mfobj##1{\@draw{##1}}%
  % axes and axis Marks:
  \def\@axes[##1]{%
    \mfcmd{axes(##1);}\@doreset}%
  \def\axes{\do@ptparam{@axes}{\the\axisheadlen}}%
  \def\@xmarks[##1]##2{%
    \mfcmd{xmarks(##1,##2);}\@doreset}%
  \def\xmarks{\do@ptparam{@xmarks}{\the\hashlen}}%
  \def\@ymarks[##1]##2{%
    \mfcmd{ymarks(##1,##2);}\@doreset}%
  \def\ymarks{\do@ptparam{@ymarks}{\the\hashlen}}%
  % points:
  \def\@point[##1]##2{%
    \if@connect
      \lines{##2}%
    \else
      \mfcmd{pointd(##1,\ifpointfilled true\else false\fi,##2);}%
    \fi
    \@doreset}%
  \def\point{\do@ptparam{@point}{\the\pointsize}}%
  % polylines:
  \def\lines##1{%
    \@draw{(curve(false, false) ##1)}}%
  % curves:
  \def\curve##1{%
    \@draw{(curve(true,false) ##1)}}%
  % cyclic curves:
  \def\cyclic##1{%
    \@draw{(curve(true,true) ##1)}}%
  % open quadratic B-splines
  \def\qspline##1{%
    \@draw{openqbs(##1)}}%
  % closed quadratic B-splines
  \def\closedqspline##1{%
    \@draw{closedqbs(##1)}}%
  % open cubic B-splines
  \def\cspline##1{%
    \@draw{opencbs(##1)}}%
  % closed cubic B-splines
  \def\closedcspline##1{%
    \@draw{closedcbs(##1)}}%
  % upright rectangles:
  \def\rect##1{%
    \@draw{rect(##1)}}%
  % circles and ellipses:
  \def\circle##1{%%
    \@draw{circle(##1)}}%
  \def\@ellipse[##1]##2{%
    \@draw{ellipse(##2,##1)}}%
  \def\ellipse{\do@ptparam{@ellipse}{0}}%
  % circular arcs:
  \def\@arc[##1]##2{%
    \if##1s\@draw{(arcpps(##2))}\else
    \if##1p\@draw{(arcplr(##2))}\else
    \if##1c\@draw{(arccps(##2))}\else
      \@draw{(arcppp(##2))}\fi\fi\fi}%
  \def\arc{\do@ptparam{@arc}{s}}%
  % polar coordinates:
  \def\@plrpoint[##1]##2{%
    \if@connect
      \plrlines{##2}%
    \else
      \mfcmd{plrpointd(##1,%
        \ifpointfilled true\else false\fi,%
        ##2);}%
    \fi
    \@doreset}%
  \def\plrpoint{\do@ptparam{@plrpoint}{\the\pointsize}}%
  \def\plrlines##1{%
    \@draw{(plrcurve(false,false) ##1)}}%
  \def\plrcurve##1{%
    \@draw{(plrcurve(true,false) ##1)}}%
  \def\plrcyclic##1{%
    \@draw{(plrcurve(true,true) ##1)}}%
  % modified polar coordinates:
  \def\turtle##1{%
    \@draw{(turtle(##1))}}%
  \def\wedge##1{%
    \@draw{(wedge(##1))}}%
  % functions:
  \def\@function[##1]##2##3{%
    \@draw{(function(%%
      \if##1s true\else false\fi, ##2, ##3))}}%
  \def\function{\do@ptparam{@function}{s}}%
  \def\@parafcn[##1]##2##3{%
    \@draw{(parafcn(
      \if##1s true\else false\fi, ##2, ##3))}}%
  \def\parafcn{\do@ptparam{@parafcn}{s}}%
  \def\@plrfcn[##1]##2##3{%
    \@draw{(plrfcn(
      \if##1s true\else false\fi, ##2, ##3))}}%
  \def\plrfcn{\do@ptparam{@plrfcn}{s}}%
  \def\@btwnfcn[##1]##2##3##4{%
    \@draw{((function(
      \if##1s true\else false\fi, ##2, ##3))
      --(reverse function(
      \if##1s true\else false\fi, ##2, ##4))
      --cycle)}}%
  \def\btwnfcn{\do@ptparam{@btwnfcn}{p}}%
  \def\@plrregion[##1]##2##3{%
    \@draw{(plrfcn(
      \if##1s true\else false\fi, ##2, ##3)
      --(0,0)--cycle)}}%
  \def\plrregion{\do@ptparam{@plrregion}{p}}%
  % end of (MF based) drawing macros.
  % (TeX based) labels and caption:
  % Labels:
  \def\@label[##1##2](##3,##4)##5{%
    % compute width of graph with label,
    % and reset size if necessary:
    \setbox\@temp=\hbox{##5}%
    % stretch graph rightwards:
    \@labeltemp=##3\mfpicunit
    \@xconv\@labeltemp
    \if##2l\advance\@labeltemp by \wd\@temp\else
    \if##2c\advance\@labeltemp by 0.5\wd\@temp\fi\fi
    \ifdim\@labeltemp>\@graphwd
      \global\@graphwd=\@labeltemp\fi
    % stretch graph leftwards:
    \@labeltemp=##3\mfpicunit
    \@xconv\@labeltemp
    \if##2r\advance\@labeltemp by -\wd\@temp\else
    \if##2c\advance\@labeltemp by -0.5\wd\@temp\fi\fi
    \ifdim\@labeltemp<\@graphleft
      \global\@graphleft=\@labeltemp\fi
    % stretch graph upwards:
    \@labeltemp=##4\mfpicunit
    \@yconv\@labeltemp
    \if##1b\advance\@labeltemp by \ht\@temp\else
    \if##1c\advance\@labeltemp by 0.5\ht\@temp\fi\fi
    \ifdim\@labeltemp>\@graphht
      \global\@graphht=\@labeltemp\fi
    % stretch graph downwards:
    \@labeltemp=##4\mfpicunit
    \@yconv\@labeltemp
    \if##1t\advance\@labeltemp by -\dp\@temp\else
    \if##1c\advance\@labeltemp by -0.5\dp\@temp\fi\fi
    \ifdim\@labeltemp<\@graphdp
      \global\@graphdp=\@labeltemp\fi
    % set label onto picture:
    \global\setbox\@labeledgraph =
      \vtop{\unvbox\@labeledgraph
        \vbox to0pt{%
          \if##1c\kern-0.5\ht\@temp\else
          \if##1b\kern-\ht\@temp\fi\fi
          \@labeltemp=##4\mfpicunit
          \@yconv\@labeltemp
          \kern\@labeltemp
          \hbox{%
            \@labeltemp=##3\mfpicunit
            \@xconv\@labeltemp
            \kern\@labeltemp
            \if##2c\kern-0.5\wd\@temp\else
            \if##2r\kern-\wd\@temp\fi\fi
            \box\@temp}%
          \vss}%
        \nointerlineskip}%
    \ignorespaces
  }% -- end \@label
  \def\label{\do@ptparam{@label}{bl}}%
  % Caption:
  % \@docaption (called by \endmfpic) :
  \def\@docaption{\global\@graphleft=0pt\relax}%
  \def\@caption[##1,##2]##3%
  {%
    % redefine \@docaption to set caption:
    \def\@docaption
    {%
      % compute adjustments to center:
      \setbox\@temp =
        \hbox\bgroup ##3\egroup
      \ifdim\wd\@temp>##1\@graphwd
        \setbox\@temp =
          \hbox
          \bgroup
            \tolerance=500\relax
            \vbox{%
              \hsize=##2\@graphwd
              \noindent ##3}%
          \egroup
      \fi
      \@centerskip=\@graphwd
      \advance\@centerskip -\wd\@temp
      \divide\@centerskip by 2
      % set caption onto picture:
      \global\setbox\@labeledgraph =
        \vbox{%
          % check if caption's wider than graph:
          \ifdim\@centerskip<0pt%
            \@graphleft = -\@centerskip
            \moveright -\@centerskip\fi
            \vbox
            \bgroup
              \unvbox\@labeledgraph
              \medskip
              \hbox{%
                \noindent
                \kern\@centerskip
                \box\@temp}%
            \egroup
            \vss}%
    }% -- end \@docaption.
  \ignorespaces
  }% -- end \@caption.
  \def\caption{\do@ptparam{@caption}{1.2,1.0}}%
  % end of object macros.
  \ignorespaces
}% -- end \@mfpic.
% restore font after reading \@mfpic.
\@tcurr
% setting up optional arguments:
\def\@pici[#1]#2#3#4#5{\@mfpic{\@param}{#1}{#2}{#3}{#4}{#5}}%
\def\mfpic[#1]{%
  \def\@param{#1}%
  \do@ptparam{@pici}{#1}}%
% ending mfpic environment:
\def\endmfpic{%
  \global\advance\@graphwd by -\@graphleft
  \global\setbox\@labeledgraph =
    \vbox
    {%
      \hbox to \@graphwd
      {%
        \kern-\@graphleft
        \box\@labeledgraph
        % \vrule height\@graphht depth-\@graphdp width 0pt
        \hss
      }% end hbox.
      \vss
    }% end vbox.
  \mfcmd{endchar;}%
  \@docaption
  \advance\@graphwd by \@graphleft
  \hbox to\@graphwd
  {%
    \kern\@graphleft
    \box\@labeledgraph
    \hss
  }% end hbox.
  \egroup
}% -- end \endmfpic.
\catcode`@=\oldatcatcode
%%%
%%%  end  mfpic.tex
%%%

